The stability of dense cores near the Serpens South protocluster

Most stars form in clusters and groups rather than in isolation. We present $\lesssim 5^{\prime\prime}$ angular resolution ($\sim 2000$ au, or 0.01 pc) Very Large Array NH$_3$ (1,1), (2,2), and (3,3) and 1.3 cm continuum emission observations of the dense gas within the Serpens South protocluster and extended filaments to the north and south. We identify 94 dense cores using a dendrogram analysis of the NH$_3$ (1,1) integrated intensity. Gas temperatures $T_K$ and non-thermal linewidths $\sigma_\mathrm{NT}$ both increase towards the centre of the young stellar cluster, in the dense gas generally and in the cores specifically. We find that most cores (54\%) are super-virial, with gravitationally bound cores located primarily in the filaments. Cores in the protocluster have higher virial parameters by a factor $\sim 1.7$, driven primarily by the increased core $\sigma_\mathrm{NT}$ values. These cores cannot collapse to form stars unless they accrete additional mass or their core internal motions are reduced. The southern filament shows a significant velocity gradient previously interpreted as mass flow toward the cluster. We find more complex kinematics in the northern filament. We find a strong correlation between $\sigma_\mathrm{NT}$ and $T_K$, and argue that the enhanced temperatures and non-thermal motions are due to mechanical heating and interaction between the protocluster-driven outflows and the dense gas. Filament-led accretion may also contribute to the increased $\sigma_\mathrm{NT}$ values. Assuming a constant fraction of core mass ends up in the young stars, future star formation in the Serpens South protocluster will shift to higher masses by a factor $\sim 2$.

==> imfit_output_table.tex <==
\begin{deluxetable*}{lcccccccc} 
\tabletypesize{\scriptsize} 
\tablecolumns{9} 
\tablewidth{0pt} 
\tablecaption{Gaussian fit results to centimeter continuum sources. \label{tab:continuum} } 
\tablehead{ 
\colhead{Source} & \colhead{Coordinates} & \colhead{Peak} & \colhead{$S_\nu$} & \colhead{$\sigma_\mathrm{maj}$} & \colhead{$\sigma_\mathrm{min}$} & \colhead{P.A.} & 
\colhead{Other names} & \colhead{Classification}\\ 
\colhead{} & \colhead{(J2000)} & \colhead{(mJy/beam)} & \colhead{(mJy)} & \colhead{(\arcsec)} & \colhead{(\arcsec)} & \colhead{(\degr)} & \colhead{} & \colhead{} 
} 
\startdata 
a & 18:30:04.13 -02:03:02.50 & 0.57 (0.04) & 1.10 (0.10) & 07.5 (00.5) & 05.6 (00.3) & 124.7 (08.1) & VLA 12\tablenotemark{a}, MM18\tablenotemark{b}, CARMA-7\tablenotemark{c} & Class 0\tablenotemark{a} \\ 
b & 18:30:03.58 -02:03:09.05 & 0.52 (0.04) & 1.18 (0.11) & 08.2 (00.6) & 06.1 (00.4) & 111.4 (08.4) & VLA 13\tablenotemark{a}, CARMA-6\tablenotemark{c} & Class 0/I\tablenotemark{a} \\ 
c & 18:30:03.35 -02:02:44.65 & 0.12 (0.03) & 0.49 (0.13) & 20.2 (06.1) & 04.5 (00.7) & 120.5 (03.0) & VLA 11\tablenotemark{a}, CARMA-5\tablenotemark{c} & Class I\tablenotemark{a} \\ 
d & 18:30:02.46 -02:02:48.19 & 0.12 (0.03) & 0.25 (0.10) & 08.3 (02.8) & 05.5 (01.4) & 169.3 (23.7) & & \\ 
e & 18:30:01.31 -02:03:42.71 & 0.32 (0.03) & 0.43 (0.07) & 05.9 (00.7) & 04.8 (00.5) & 119.1 (18.8) & VLA 17\tablenotemark{a} & Flat/Class II\tablenotemark{a} \\ 
f & 18:30:05.87 -02:01:44.57 & 0.14 (0.03) & 0.31 (0.10) & 11.4 (03.4) & 04.2 (00.6) & 95.0 (05.2) & VLA 7\tablenotemark{a} & Class II\tablenotemark{a} \\ 
g & 18:30:09.65 -02:00:33.44 & 0.16 (0.03) & 0.25 (0.08) & 07.5 (01.9) & 04.5 (00.8) & 147.1 (13.0) & VLA 1\tablenotemark{a} & Extragal.\tablenotemark{a} \\ 
h & 18:30:01.56 -02:00:51.31 & 0.19 (0.04) & 0.31 (0.09) & 07.0 (01.5) & 05.1 (00.8) & 46.0 (20.1) & & \\ 
i & 18:30:15.03 -02:08:07.68 & 0.15 (0.03) & 0.26 (0.08) & 08.6 (02.4) & 04.2 (00.7) & 82.7 (08.5) & & \\ 
\enddata 
%\tablecomments{}
\tablerefs{$^{a}$ \citet{kern_2016}; $^b$ \citet{maury_2011}; $^c$ \citet{plunkett_2015_outflows}}
\end{deluxetable*}
